Detecting Gang-Involved Escalation on Social Media Using Context

Gang-involved youth in cities such as Chicago have increasingly turned to social media to post about their experiences and intents online. In some situations, when they experience the loss of a loved one, their online expression of emotion may evolve into aggression towards rival gangs and ultimately into real-world violence. In this paper, we present a novel system for detecting Aggression and Loss in social media. Our system features the use of domain-specific resources automatically derived from a large unlabeled corpus, and contextual representations of the emotional and semantic content of the user's recent tweets as well as their interactions with other users. Incorporating context in our Convolutional Neural Network (CNN) leads to a significant improvement.

==> Abstract.tex <==
\begin{abstract}
\end{abstract}

==> Methods_CNN.tex <==
\subsection{CNN Baseline}

We begin with definitions of terms before defining our baseline
CNN model. Let $[a] = {1, 2, \ldots, a}$ be the sequence 
from 1 to $a$ for any positive 
integer $a$.
Let $|a|$ be the
cardinality of $a$ when applied to a set or sequence and the  absolute value when $a$ is a scalar.
Let a tweet $\tweet = \{\tweet_1, \ldots, \tweet_n\}$ be an ordered 
sequence of $n$ tokens\footnote{
These tokens can either be at the word or character level; 
where the distinction between word or character is irrelevant to the model
description, we use the term ``token.''}.
Each token is drawn from a vocabulary $\Vocab$ with which we associate 
an embedding matrix $\embw \in \mathbb{R}^{|\Vocab| \times d}.$
%Each row in $\embw$ is a $d$-dimensional embedding corresponding to an 
%entry in the vocabulary where $W_{c_i}$ indicates the embedding
%associated with the token $c_i$.
%We define the function
%$\embf(\tweet) = [\embw_{\tweet_1}, \embw_{\tweet_2}, \ldots,
%\embw_{\tweet_n}]$ as the concatentation of the embeddings 
%associated with the tokens $\tweet_i$ into an
%$n \times d$ matrix for any tweet $\tweet$.
%Given parameters $\convw \in \mathbb{R}^{w\times d}$ and 
%$b \in \mathbb{R}$, 
The space of classification labels $\mathcal{Y} = \{\textit{Other}, \;\textit{Loss}, \;\textit{Aggression}\}$. We refer to \textit{Aggression} as `A' and similarly \textit{Loss} as `L' wherever unambiguous.


We define CNN with filter widths
$w \in [M]$, where $M$ is the maximum filter size, and $F$ filters per width. Our architecture is defined as:
\begin{align*}
X & = \embf(c)\\
A^{w} & = Conv1D(X) \ \forall w \in [M]\\
B^{w} & = MaxPool1D(A^{w})\\
%a^{(w,f)}_{i} & = \convb^{(w,f)} +\sum_{j \in [w], k\in [d]}
%\convw^{(w,f)}_{j,k}\cdot X_{i+j,k} \\
%h^{(w,f)} & =\max_{i \in [|c|-w + 1]} 
%\textsc{ReLU}\left(a^{(w,f)}_{i}\right)\\
r &= \left[B^{w} \ \forall w \in [M]\right]\\
h & = Dense(r)\\
p & = \textsc{Sigmoid}(Vh + b)
\end{align*}
Here $X \in \mathbb{R}^{|c|\times d}$, $A^{w} \in \mathbb{R}^{(|c|-w+1)\times F}$, $B^{w} \in \mathbb{R}^{F}$, $r\in \mathbb{R}^{MF}$, $h \in \mathbb{R}^{256}$ and $p$ is the probability of the positive class. Further, $\embf$ means the embedding layer, $Conv1D$ means 1-D convolution, $MaxPool1D$ means global 1-D max pooling, and $Dense$ means dense layer. 

We train two one-vs-rest CNN classifiers for classes \textit{Aggression} and \textit{Loss} respectively. We don't train a CNN classifier for the \textit{Other} class. We perform 3-way classification by first classifying the tweet as \textit{Aggression} if the output probability $p(y = A|c;\Theta_{A})$ exceeds threshold $t_{A}$. Next we classify the yet unclassified tweets as \textit{Loss} if the output probability $p(y = L|c;\Theta_{L})$ exceeds threshold $t_{L}$. Finally the yet unclassified tweets are classified as \textit{Other}. The thresholds $t_{A}$ and $t_{L}$ are tuned on the validation set to maximize the f-score of \textit{Aggression} and \textit{Loss} respectively.
Given our labeled training data, $\mathcal{D} = \{(c^{(i)}, y^{(i)} )\}_{i=1}^N,$ we fit the parameters $\Theta$ by
minimizing the negative log likelihood 
$-\frac{1}{N}\sum_{i=1}^N \log p\left(y^{(i)}|c^{(i)};\Theta\right)$ using the Adam optimizer and early stopping on the validation set using validation loss as the stopping criterion.
For the CNN classifiers, we use the following hyperparameters: kernel size up to $M = 2$, dense layer dimension $F = 200$, \textit{ReLU} activation in $Conv1D$ and $Dense$ layers, and 50\% Dropout is applied after $\embf$ and $Conv1D$ layers, respectively.

 For the baseline CNN classifier 
 %and the distantly labeled pre-training method, 
 we experiment with both word and character level inputs. Whereas word level models can more easily incorporate direct semantic information about the content of the tweet via word embeddings, character-level models can bypass many of the restrictions encountered at the word level to identify more salient information, including variations on spelling of certain words, as well as any important signals embedded in long, one-off hashtag phrases that are difficult to tokenize properly.
 
We incorporate context information into the neural network in the following way. Each type of context features takes the form of a real vector: i) both {\em word embedding user history} and {\em word embedding user interaction} features are in $\mathbb{R}^{300}$ and ii) {\em splex user history} features are in $\mathbb{R}^{2}$. We concatenate these feature vectors with the last layer $h$ before the final classification output. 

%We incorporate user information in a similar way. For a given tweet, suppose user $u_{post}$ posts the tweet, $u_{rt}$ is the user being retweeted and $u_{mention}$ is the user who is mentioned. We map each of $u_{post}, u_{rt}, u_{mention}$ to 300 dimensional real vector $f_{u_{post}}, f_{u_{rt}}, f_{u_{mention}} \in \mathbb{R}^{300}$ by using an user embedding matris $E$. After that, each of $f_{u_{post}}, f_{u_{rt}}, f_{u_{mention}}$ is concatenated to the last layer $h$ just as other context feature vectors. For tweets that are not retweets/no users are mentioned, $f_{u_{rt}}$/$f_{u_{mention}}$ is 0.  

\eanote{Reviewer 1 asked for more detail on the CNN's filter sizes and dropout. This is included in Supplementary.tex, but maybe should also be included here?}
 
% We are now ready to define our baseline CNN
% classifier, which is composed of two parts, the $\ConvNet$ 
% feature extractor with parameters $\Psi$ 
% and the multi-layer perceptron $\mlp$ with parameters $\Phi$.
% I.e., the class probabilities of a tweet $c$ are  
% defined $p(y=i|c; \Theta) = \mlp(\ConvNet(c))_i$ and the model
% has dependence on parameters $\Theta = \{\Psi, \Phi \}.$

% Given our labeled training data, $\mathcal{D} = \{(c^{(i)}, y^{(i)} )\}_{i=1}^N,$ we fit the parameters $\Theta$ by
% minimizing the negative log likelihood: 
% $-\frac{1}{N}\sum_{i=1}^N \log p\left(y^{(i)}|c^{(i)};\Theta\right)$ using 
% the Nesterov Adam optimizer available in Keras and early stopping on the labeled validation set.


%  For the baseline CNN classifier and the distantly 
%  labeled pre-training methods, we experiment with both
%  word and character level inputs. Whereas word level models can more easily incorporate direct semantic information about the content of the tweet via word embeddings, character-level models can bypass many of the restrictions encountered at the word level to identify more salient information, including variations on spelling of certain words, as well as any important signals embedded
%  in long, one-off hashtag phrases that are difficult to
%  tokenize properly.
%  The character level model is less well motivated 
%  for our CFP method and so we only run that model at 
%  the word level.
 


